Leveraging Adiabatic Quantum Computation for Election Forecasting

Accurate, reliable sampling from fully-connected graphs with arbitrary correlations is a difficult problem. Such sampling requires knowledge of the probabilities of observing every possible state of a graph. As graph size grows, the number of model states becomes intractably large and efficient computation requires full sampling be replaced with heuristics and algorithms that are only approximations of full sampling. This work investigates the potential impact of adiabatic quantum computation for sampling purposes, building on recent successes training Boltzmann machines using a quantum device. We investigate the use case of quantum computation to train Boltzmann machines for predicting the 2016 Presidential election.

==> h-physrev <==
ENTRY
{ address
eprint
author
booktitle
chapter
collaboration
edition
editor
howpublished
institution
journal
key
month
note
number
organization
pages
publisher
school
series
title
type
volume
year
}
{}
{ label }
INTEGERS { output.state before.all mid.sentence after.sentence after.block }
FUNCTION {init.state.consts}
{ #0 'before.all :=
#1 'mid.sentence :=
#2 'after.sentence :=
#3 'after.block :=
}
STRINGS { s t }
FUNCTION {output.nonnull}
{ 's :=
output.state mid.sentence =
{ ", " * write$ }
{ output.state after.block =
{ "," * write$
newline$
"\newblock " write$
}
{ output.state before.all =
'write$
{ add.period$ " " * write$ }
if$
}
if$
mid.sentence 'output.state :=
}
if$
s
}
FUNCTION {output}
{ duplicate$ empty$
'pop$
'output.nonnull
if$
}
FUNCTION {output.check}
{ 't :=
duplicate$ empty$
{ pop$ "empty " t * " in " * cite$ * warning$ }
'output.nonnull
if$
}
FUNCTION {output.bibitem}
{ newline$
"\bibitem{" write$
cite$ write$
"}" write$
newline$
""
before.all 'output.state :=
}
FUNCTION {fin.entry}
{ add.period$
write$
newline$
}
FUNCTION {new.block}
{ output.state before.all =
'skip$
{ after.block 'output.state := }
if$
}
FUNCTION {new.sentence}
{ skip$
}
FUNCTION {not}
{   { #0 }
{ #1 }
if$
}
FUNCTION {and}
{   'skip$
{ pop$ #0 }
if$
}
FUNCTION {or}
{   { pop$ #1 }
'skip$
if$
}
FUNCTION {new.block.checka}
{ empty$
'skip$
'new.block
if$
}
FUNCTION {new.block.checkb}
{ empty$
swap$ empty$
and
'skip$
'new.block
if$
}
FUNCTION {new.sentence.checka}
{ empty$
'skip$
'new.sentence
if$
}
FUNCTION {new.sentence.checkb}
{ empty$
swap$ empty$
and
'skip$
'new.sentence
if$
}
FUNCTION {field.or.null}
{ duplicate$ empty$
{ pop$ "" }
'skip$
if$
}
FUNCTION {emphasize}
{ duplicate$ empty$
{ pop$ "" }
{ "{\em " swap$ * "}" * }
if$
}
FUNCTION {embolden}
{ duplicate$ empty$
{ pop$ "" }
{ "{\bf " swap$ * "}" * }
if$
}
FUNCTION {paren}
{ duplicate$ empty$
{ pop$ "" }
{ "(" swap$ * ")" * }
if$
}
INTEGERS { nameptr namesleft numnames }
INTEGERS { etal }
FUNCTION {format.names}
{ 's :=
#1 'nameptr :=
s num.names$ 'numnames :=
numnames #5 >
s numnames "{ll}" format.name$ "others" = numnames #1 > and
or 'etal :=
etal
{ #1 #1 + 'namesleft := }
{ numnames 'namesleft := }
if$
{ namesleft #0 > }
{ s nameptr "{f.~}{vv~}{ll}{, jj}" format.name$ 't :=
nameptr #1 >
{ namesleft #1 >
{ ", " * t * }
{ nameptr #2 >
{ "," * }
'skip$
if$
t "others" =
etal or
{ " {\em et~al.}" * }
{ " and " * t * }
if$
}
if$
}
't
if$
nameptr #1 + 'nameptr :=
namesleft #1 - 'namesleft :=
}
while$
}
FUNCTION {format.authors}
{ author empty$
{ "" }
{ author format.names }
if$
}
FUNCTION {format.editors}
{ editor empty$
{ "" }
{ editor format.names
editor num.names$ #1 >
{ ", editors" * }
{ ", editor" * }
if$
}
if$
}
FUNCTION {format.edited}
{ editor empty$
{ "" }
{ "edited by " editor format.names * }
if$
}
FUNCTION {format.title}
{ title empty$
{ "" }
{ title "t" change.case$ }
if$
}
FUNCTION {n.dashify}
{ 't :=
""
{ t empty$ not }
{ t #1 #1 substring$ "-" =
{ t #1 #2 substring$ "--" = not
{ "--" *
t #2 global.max$ substring$ 't :=
}
{   { t #1 #1 substring$ "-" = }
{ "-" *
t #2 global.max$ substring$ 't :=
}
while$
}
if$
}
{ t #1 #1 substring$ *
t #2 global.max$ substring$ 't :=
}
if$
}
while$
}
FUNCTION {first.page}
{ 't :=
""
{  t empty$ not t #1 #1 substring$ "-" = not and }
{ t #1 #1 substring$ *
t #2 global.max$ substring$ 't :=
}
while$
}
FUNCTION {format.date}
{ year empty$
{ "" }
'year
if$
}
FUNCTION {format.btitle}
{ title emphasize
}
FUNCTION {tie.or.space.connect}
{ duplicate$ text.length$ #3 <
{ "~" }
{ " " }
if$
swap$ * *
}
FUNCTION {either.or.check}
{ empty$
'pop$
{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
if$
}
FUNCTION {format.bvolume}
{ volume empty$
{ "" }
{ series empty$
'skip$
{ ", " series * }
if$
" Vol." volume tie.or.space.connect *
"volume and number" number either.or.check
}
if$
}
FUNCTION {format.number.series}
{ volume empty$
{ number empty$
{ series field.or.null }
{  series empty$
{ "there's a number but no series in " cite$ * warning$ }
{ ", " series * }
if$
" No. " number tie.or.space.connect *
}
if$
}
{ "" }
if$
}
FUNCTION {format.edition}
{ edition empty$
{ "" }
{ output.state mid.sentence =
{ ", " edition "l" change.case$ *  }
{ ", " edition "t" change.case$ *  }
if$
" ed." *
}
if$
}
INTEGERS { multiresult }
FUNCTION {multi.page.check}
{ 't :=
#0 'multiresult :=
{ multiresult not
t empty$ not
and
}
{ t #1 #1 substring$
duplicate$ "-" =
swap$ duplicate$ "," =
swap$ "+" =
or or
{ #1 'multiresult := }
{ t #2 global.max$ substring$ 't := }
if$
}
while$
multiresult
}
FUNCTION {format.pages}
{ pages empty$
{ "" }
{ pages multi.page.check
{ "pp." pages n.dashify tie.or.space.connect }
{ "p." pages tie.or.space.connect }
if$
}
if$
}
FUNCTION {format.pages.a}
{ pages empty$
{ "" }
{ "p." pages first.page tie.or.space.connect }
if$
}
FUNCTION {format.vol.num.pages}
{ volume field.or.null embolden
" " swap$ * *
pages empty$
'skip$
{ duplicate$ empty$
{ pop$ format.pages.a }
{ ", " * pages first.page * }
if$
}
if$
}
FUNCTION {format.chapter.pages}
{ chapter empty$
'format.pages
{ type empty$
{ "chap." }
{ type "l" change.case$ }
if$
chapter tie.or.space.connect
pages empty$
'skip$
{ ", " * format.pages * }
if$
}
if$
}
FUNCTION {format.pub.addr.date}
{ publisher empty$
{ "" "empty publisher in " cite$ * warning$ }
{ publisher
address empty$
'skip$
{ ", " * address * }
if$
}
if$
year empty$
{ "empty year in " cite$ * warning$ }
{ ", " * year * }
if$
paren " " swap$ *
}
FUNCTION {format.book.entry}
{ format.btitle
format.bvolume *
format.number.series *
format.edition *
format.pub.addr.date *
}
FUNCTION {format.inbook.entry}
{ format.book.entry
", " *
format.chapter.pages *
}
FUNCTION {format.in.ed.booktitle}
{ booktitle empty$
{ "" }
{ editor empty$
{ "in " booktitle emphasize * }
{ "in " booktitle emphasize * ", " * format.edited * }
if$
}
if$
}
FUNCTION {empty.misc.check}
{ author empty$ title empty$ howpublished empty$
month empty$ year empty$ note empty$
and and and and and
{ "all relevant fields are empty in " cite$ * warning$ }
'skip$
if$
}
FUNCTION {format.thesis.type}
{ type empty$
'skip$
{ pop$
type "t" change.case$
}
if$
}
FUNCTION {format.inst.tr.num.date}
{ institution empty$
{ "" "empty institution in " cite$ * warning$ }
{ institution }
if$
" Report No." *
number empty$
{ "" }
{ number tie.or.space.connect }
if$
year empty$
{ "empty year in " cite$ * warning$ }
{ ", " * year * " (unpublished)" * }
if$
}
FUNCTION {format.article.crossref}
{ key empty$
{ journal empty$
{ "need key or journal for " cite$ * " to crossref " * crossref *
warning$
""
}
{ "In " journal * }
if$
}
{ "In " key * }
if$
" \cite{" * crossref * "}" *
}
FUNCTION {format.crossref.editor}
{ editor #1 "{vv~}{ll}" format.name$
editor num.names$ duplicate$
#2 >
{ pop$ " {\em et~al.}" * }
{ #2 <
'skip$
{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
{ " {\em et~al.}" * }
{ " and " * editor #2 "{vv~}{ll}" format.name$ * }
if$
}
if$
}
if$
}
FUNCTION {format.book.crossref}
{ volume empty$
{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
"In "
}
{ "Volume" volume tie.or.space.connect
" of " *
}
if$
editor empty$
editor field.or.null author field.or.null =
or
{ key empty$
{ series empty$
{ "need editor, key, or series for " cite$ * " to crossref " *
crossref * warning$
"" *
}
{ "{\em " * series * "\/}" * }
if$
}
{ key * }
if$
}
{ format.crossref.editor * }
if$
" \cite{" * crossref * "}" *
}
FUNCTION {format.incoll.inproc.crossref}
{ editor empty$
editor field.or.null author field.or.null =
or
{ key empty$
{ booktitle empty$
{ "need editor, key, or booktitle for " cite$ * " to crossref " *
crossref * warning$
""
}
{ "In {\em " booktitle * "\/}" * }
if$
}
{ "In " key * }
if$
}
{ "In " format.crossref.editor * }
if$
" \cite{" * crossref * "}" *
}
FUNCTION {article}
{ output.bibitem
collaboration output
format.authors "author" output.check
new.block
crossref missing$
{ journal field.or.null
format.vol.num.pages 
format.date empty$
'skip$
{ duplicate$ empty$
{ pop$ format.date paren }
{ " " * format.date paren * }
if$
}
if$
output
}
{ format.article.crossref output.nonnull
format.pages output
}
if$
eprint output
new.block
note output
fin.entry
}
FUNCTION {book}
{ output.bibitem
collaboration output
author empty$
{ format.editors "author and editor" output.check }
{ format.authors output.nonnull
crossref missing$
{ "author and editor" editor either.or.check }
'skip$
if$
}
if$
new.block
crossref missing$
{ format.book.entry output }
{ new.block
format.book.crossref output.nonnull
}
if$    
eprint output
new.block
note output
fin.entry
}
FUNCTION {booklet}
{ output.bibitem
collaboration output
format.authors output
new.block
format.title "title" output.check
howpublished address new.block.checkb
howpublished output
address output
format.date output
eprint output
new.block
note output
fin.entry
}
FUNCTION {inbook}
{ output.bibitem
collaboration output
author empty$
{ format.editors "author and editor" output.check }
{ format.authors output.nonnull
crossref missing$
{ "author and editor" editor either.or.check }
'skip$
if$
}
if$
new.block
crossref missing$
{ format.inbook.entry output }
{ format.chapter.pages "chapter and pages" output.check
new.block
format.book.crossref output.nonnull
}
if$
eprint output
new.block
note output
fin.entry
}
FUNCTION {incollection}
{ output.bibitem
collaboration output
format.authors "author" output.check
new.block
format.title "title" output.check
new.block
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
format.bvolume output
format.number.series output
format.chapter.pages output
new.sentence
publisher "publisher" output.check
address output
format.edition output
format.date "year" output.check
}
{ format.incoll.inproc.crossref output.nonnull
format.chapter.pages output
}
if$
eprint output
new.block
note output
fin.entry
}
FUNCTION {inproceedings}
{ output.bibitem
collaboration output
format.authors "author" output.check
new.block
format.title "title" output.check
new.block
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
format.bvolume output
format.number.series output
format.pages output
address empty$
{ organization publisher new.sentence.checkb
organization output
publisher output
format.date "year" output.check
}
{ address output.nonnull
format.date "year" output.check
new.sentence
organization output
publisher output
}
if$
}
{ format.incoll.inproc.crossref output.nonnull
format.pages output
}
if$
eprint output
new.block
note output
fin.entry
}
FUNCTION {conference} { inproceedings }
FUNCTION {manual}
{ output.bibitem
collaboration output
author empty$
{ organization empty$
'skip$
{ organization output.nonnull
address output
}
if$
}
{ format.authors output.nonnull }
if$
new.block
format.btitle "title" output.check
author empty$
{ organization empty$
{ address new.block.checka
address output
}
'skip$
if$
}
{ organization address new.block.checkb
organization output
address output
}
if$
format.edition output
format.date output
eprint output
new.block
note output
fin.entry
}
FUNCTION {mastersthesis}
{ output.bibitem
format.authors "author" output.check
new.block
format.title "title" output.check
new.block
"Master's thesis" format.thesis.type output.nonnull
school "school" output.check
address output
format.date "year" output.check
eprint output
new.block
note output
fin.entry
}
FUNCTION {misc}
{ output.bibitem
collaboration output
format.authors output
title howpublished new.block.checkb
format.title output
howpublished new.block.checka
howpublished output
format.date output
eprint output
new.block
note output
fin.entry
empty.misc.check
}
FUNCTION {phdthesis}
{ output.bibitem
format.authors "author" output.check
new.block
format.btitle "title" output.check
new.block
"PhD thesis" format.thesis.type output.nonnull
school "school" output.check
address output
format.date "year" output.check
eprint output
new.block
note output
fin.entry
}
FUNCTION {proceedings}
{ output.bibitem
collaboration output
editor empty$
{ organization output }
{ format.editors output.nonnull }
if$
new.block
format.btitle "title" output.check
format.bvolume output
format.number.series output
address empty$
{ editor empty$
{ publisher new.sentence.checka }
{ organization publisher new.sentence.checkb
organization output
}
if$
publisher output
format.date "year" output.check
}
{ address output.nonnull
format.date "year" output.check
new.sentence
editor empty$
'skip$
{ organization output }
if$
publisher output
}
if$
eprint output
new.block
note output
fin.entry
}
FUNCTION {techreport}
{ output.bibitem
collaboration output
format.authors "author" output.check
new.block
format.inst.tr.num.date output.nonnull
eprint output
new.block
note output
fin.entry
}
FUNCTION {unpublished}
{ output.bibitem
collaboration output
format.authors "author" output.check
new.block
format.title "title" output.check
new.block
note "note" output.check
format.date output
fin.entry
}
FUNCTION {default.type} { misc }
MACRO {jan} {"Jan."}
MACRO {feb} {"Feb."}
MACRO {mar} {"Mar."}
MACRO {apr} {"Apr."}
MACRO {may} {"May"}
MACRO {jun} {"June"}
MACRO {jul} {"July"}
MACRO {aug} {"Aug."}
MACRO {sep} {"Sept."}
MACRO {oct} {"Oct."}
MACRO {nov} {"Nov."}
MACRO {dec} {"Dec."}
MACRO {acmcs} {"ACM Comput. Surv."}
MACRO {acta} {"Acta Inf."}
MACRO {cacm} {"Commun. ACM"}
MACRO {ibmjrd} {"IBM J. Res. Dev."}
MACRO {ibmsj} {"IBM Syst.~J."}
MACRO {ieeese} {"IEEE Trans. Softw. Eng."}
MACRO {ieeetc} {"IEEE Trans. Comput."}
MACRO {ieeetcad}
{"IEEE Trans. Comput.-Aided Design Integrated Circuits"}
MACRO {ipl} {"Inf. Process. Lett."}
MACRO {jacm} {"J.~ACM"}
MACRO {jcss} {"J.~Comput. Syst. Sci."}
MACRO {scp} {"Sci. Comput. Programming"}
MACRO {sicomp} {"SIAM J. Comput."}
MACRO {tocs} {"ACM Trans. Comput. Syst."}
MACRO {tods} {"ACM Trans. Database Syst."}
MACRO {tog} {"ACM Trans. Gr."}
MACRO {toms} {"ACM Trans. Math. Softw."}
MACRO {toois} {"ACM Trans. Office Inf. Syst."}
MACRO {toplas} {"ACM Trans. Prog. Lang. Syst."}
MACRO {tcs} {"Theoretical Comput. Sci."}
MACRO {advp} {"Adv. Phys."}
MACRO {ajp} {"Am. J. Phys."}
MACRO {ao} {"Appl. Opt."}
MACRO {apj} {"Astrophys. J."}
MACRO {apl} {"Appl. Phys. Lett."}
MACRO {arnps} {"Ann. Rev. Nucl. Sci."}
MACRO {arns} {"Ann. Rev. Nucl. Part. Sci."}
MACRO {baps} {"Bull. Am. Phys. Soc."}
MACRO {cpc} {"Computer Phys. Comm."}
MACRO {cppcf} {"Comments Plasma Phys. Controlled Fusion"}
MACRO {fed} {"Fusion Eng. Design"}
MACRO {ft} {"Fusion Tech."}
MACRO {ieeens} {"IEEE Trans. Nucl. Sci."}
MACRO {ieeeps} {"IEEE Trans. Plasma Sci."}
MACRO {ijimw} {"Int. J. Infrared Millimeter Waves"}
MACRO {ip} {"Infrared Phys."}
MACRO {jap} {"J. Appl. Phys."}
MACRO {jcp} {"J. Comput. Phys."}
MACRO {jetp} {"Sov. Phys.-JETP"}
MACRO {jfe} {"J. Fusion Energy"}
MACRO {jfm} {"J. Fluid Mech."}
MACRO {jgr} {"J. Geophys. Res."}
MACRO {jmp} {"J. Math. Phys."}
MACRO {jne} {"J. Nucl. Energy"}
MACRO {jnm} {"J. Nucl. Mater."}
MACRO {josa} {"J. Opt. Soc. Am."}
MACRO {jpg} {"J. Phys.~G: Nucl. and Part. Phys."}
MACRO {jphys} {"J. Phys"}
MACRO {jpp} {"J. Plasma Phys."}
MACRO {jpsj} {"J. Phys. Soc. Jpn"}
MACRO {jvst} {"J. Vac. Sci. Technol."}
MACRO {modphyslettA} {"Mod. Phys. Lett. A"}
MACRO {nedf} {"Nucl. Eng. Design/Fusion"}
MACRO {nf} {"Nucl. Fusion"}
MACRO {nim} {"Nucl. Instrum. Methods"}
MACRO {np} {"Nucl. Phys."}
MACRO {npb} {"Nucl. Phys.~B"}
MACRO {npbps} {"Nucl. Phys. B (Proc. Suppl.)"}
MACRO {nt/f} {"Nucl. Tech./Fusion"}
MACRO {pf} {"Phys. Fluids"}
MACRO {pl} {"Phys. Lett."}
MACRO {plb} {"Phys. Lett.~B"}
MACRO {pnas} {"Proc. Nat. Acad. Sci. USA"}
MACRO {pp} {"Plasma Phys."}
MACRO {physrep} {"Phys. Rep."}
MACRO {physrev} {"Phys. Rev."}
MACRO {pr} {"Phys. Rev."}
MACRO {prd} {"Phys. Rev.~D"}
MACRO {prl} {"Phys. Rev. Lett."}
MACRO {procroysoc} {"Proc. Roy. Soc"}
MACRO {ps} {"Physica Scripta"}
MACRO {rmp} {"Rev. Mod. Phys."}
MACRO {rsi} {"Rev. Sci. Instrum."}
MACRO {sjnp} {"Sov. J. Nucl. Phys."}
MACRO {sjpp} {"Sov. J. Plasma Phys."}
MACRO {spd} {"Sov. Phys.-Dokl."}
MACRO {sptp} {"Sov. Phys.-Tech. Phys."}
MACRO {spu} {"Sov. Phys.-Usp."}
MACRO {zp} {"Z. Phys."}
MACRO {zpc} {"Z. Phys.~C"}
READ
STRINGS { longest.label }
INTEGERS { number.label longest.label.width }
FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
#1 'number.label :=
#0 'longest.label.width :=
}
FUNCTION {longest.label.pass}
{ number.label int.to.str$ 'label :=
number.label #1 + 'number.label :=
label width$ longest.label.width >
{ label 'longest.label :=
label width$ 'longest.label.width :=
}
'skip$
if$
}
EXECUTE {initialize.longest.label}
ITERATE {longest.label.pass}
FUNCTION {begin.bib}
{ preamble$ empty$
'skip$
{ preamble$ write$ newline$ }
if$
"\begin{thebibliography}{"  longest.label  * "}" * write$ newline$
}
EXECUTE {begin.bib}
EXECUTE {init.state.consts}
ITERATE {call.type$}
FUNCTION {end.bib}
{ newline$
"\end{thebibliography}" write$ newline$
}
EXECUTE {end.bib}

